Undecidability of future timeline-based planning over dense temporal domains

Planning is one of the most studied problems in computer science. In this paper, we consider the timeline-based approach, where the domain is modeled by a set of independent, but interacting, components, identified by a set of state variables, whose behavior over time (timelines) is governed by a set of temporal constraints (synchronization rules). Timeline-based planning in the dense-time setting has been recently shown to be undecidable in the general case, and undecidability relies on the high expressiveness of the trigger synchronization rules. In this paper, we strengthen the previous negative result by showing that undecidability already holds under the future semantics of the trigger rules which limits the comparison to temporal contexts in the future with respect to the trigger.

==> abstract.tex <==
In this paper, we address complexity issues for timeline-based planning over dense temporal domains.
%Planning is one of the most studied problems in computer science. In the timeline-based approach, 
The planning problem is modeled by means of a set of independent, but interacting, components, each one represented by a number of state variables, whose behavior over time (timelines) is governed by a set of temporal constraints (synchronization rules).
While the temporal domain is usually assumed to be discrete, here we consider the dense case.  
%only recently the planning problem has been addressed in the dense domain showing that 
Dense timeline-based planning has been recently shown to be undecidable in the general case; decidability (NP-completeness) can be recovered by restricting to purely existential synchronization rules (\emph{trigger-less rules}).
In this paper, we investigate the unexplored area of intermediate cases in between these two extremes.
%the above two boundaries.
We first show that \textbf{decidability} and \textbf{non-primitive recursive hardness} can be proved by admitting synchronization rules with a trigger, but forcing them to suitably check constraints only in the future with respect to the trigger (\emph{future simple rules}). More \lq\lq tractable\rq\rq{}
%hardness 
results can be obtained by additionally constraining the form of intervals in future 
%one-only synchronization 
simple rules: 
%(i) $\EXPSPACE$-hardness 
$\EXPSPACE$-completeness is guaranteed by avoiding singular intervals, 
%and (ii) $\Psp$-hardness 
 $\Psp$-completeness by admitting only intervals of the forms $[0,a]$ and $[b,+\infty[$.

==> concl.tex <==
\section{Conclusion}
In this paper, we investigated decidability and complexity issues for TP over dense temporal domains. Such a problem is known to be undecidable~\cite{techrep} even if restricted to simple trigger rules. Here, we have shown that decidability can be recovered by adding the future semantics to simple trigger rules.
Moreover, future TP with simple trigger rules has been proved to be non-primitive recursive-hard 
(the same result holds in the case of future TP with all intervals being in $\Intv_{(0,\infty)}$).
Finally, if, additionally, singular intervals are avoided, it turns out to be $\EXPSPACE$-complete, 
and $\Psp$-complete if we consider only intervals in $\Intv_{(0,\infty)}$.
%
Future work will focus on decidability of future TP with arbitrary trigger rules which remains open.
